Transfer learning of phase transitions in percolation and directed percolation

The latest advances of statistical physics have shown remarkable performance of machine learning in identifying phase transitions. In this paper, we apply domain adversarial neural network (DANN) based on transfer learning to studying non-equilibrium and equilibrium phase transition models, which are percolation model and directed percolation (DP) model, respectively. With the DANN, only a small fraction of input configurations (2d images) needs to be labeled, which is automatically chosen, in order to capture the critical point. To learn the DP model, the method is refined by an iterative procedure in determining the critical point, which is a prerequisite for the data collapse in calculating the critical exponent $\nu_{\perp}$. We then apply the DANN to a two-dimensional site percolation with configurations filtered to include only the largest cluster which may contain the information related to the order parameter. The DANN learning of both models yields reliable results which are comparable to the ones from Monte Carlo simulations. Our study also shows that the DANN can achieve quite high accuracy at much lower cost, compared to the supervised learning.

==> Flow1.tikz.tex <==
%\usetikzlibrary{arrows.meta}
\usetikzlibrary{positioning,calc}
\usetikzlibrary{arrows}
\tikzset{%
%  >={Latex[width=2mm,length=2mm]},
  % Specifications for style of nodes:
      base/.style = {rectangle, rounded corners, draw=black,
                           minimum width=4cm, minimum height=1cm,
                           text centered, font=\sffamily},
       activityStarts/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2cm, minimum height=1.5cm,
                           text centered, font=\sffamily, fill=white!30},
       latent/.style = {ellipse, rounded corners, draw=black,
                           minimum width=0.1cm, minimum height=2cm,
                           text centered, font=\sffamily, fill=orange!20},
       feature/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.5cm, minimum height=2cm,
                           text centered, font=\sffamily,fill=green!30},
       LP/.style = {rectangle, rounded corners, draw=black,
                           minimum width=3.1cm, minimum height=1cm,
                           text centered, font=\sffamily, fill=blue!30},
       DC/.style = {rectangle, rounded corners, draw=black,
                           minimum width=1.5cm, minimum height=1cm,
                           text centered, font=\sffamily, fill=red!30},
       yd/.style = {rectangle, rounded corners, draw=black,
                           minimum width=2.1cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=white!30},
        Ly/.style = {rectangle, rounded corners, draw=blue!60, line width=0.5mm,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=white!30},
        Ld/.style = {rectangle, rounded corners, draw=red!60, line width=0.5mm,
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=white!30},

    activityRuns/.style = {rectangle, rounded corners, draw=black, 
                           minimum width=0.5cm, minimum height=0.5cm,
                           text centered, font=\sffamily, fill=green!30},
         process/.style = {base, minimum width=2.5cm, fill=blue!15,
                           font=\ttfamily},
      functions/.style = {rectangle, rounded corners, draw=black,
                           minimum width=0.5cm, minimum height=1cm,
                           text centered, font=\sffamily, fill=yellow!30},
}


\def\layersep{2.5cm}
\def\nodeinlayersep{1.5cm}
\resizebox{1\textwidth}{!}{% 
\begin{tikzpicture}[node distance=2cm,
    every node/.style={fill=white, font=\sffamily}, align=center]
  % Specification of nodes (position, etc.)
  \coordinate (input);
  \node (LB)             [activityStarts]              {\footnotesize Source\\\footnotesize Domain};
 % \node (Encoder1)     [process, right= 5mm of LB]          {Encoder 1};
  %\node (es1)      [activityStarts1,  right= 5mm of Encoder1]   {$\mu$, $\sigma$,\\$\pi$};
   \node (ULB)     [activityStarts, below of=LB]   {\footnotesize Target\\ \footnotesize Domain};
   % \node (Encoder2)     [process, below of=Encoder1]          {Encoder 2};
   % \node (es2)      [activityStarts1, right= 5mm of Encoder2]   {$\mu${\scriptsize$'$}, $\sigma${\scriptsize$'$},\\$\pi${\scriptsize$'$}};
 %  \node (onResumeBlock)     [activityStarts, right of =es1]   {z\\z\\z\\z\\z};
   \node (Feature)  [ feature, right= 1.5 cm of {$(LB)!0.5!(ULB)$}]   {\large Feature extractor \\  \footnotesize CNN+Max-pooling+flatten+sigmoid+ \\ \footnotesize FC(500)+BN+dropout+sigmoid} ; 
   \node (Latent) [ latent, right = 0.5 cm of Feature]  {\footnotesize Latent  \\ \footnotesize variables \\ \footnotesize(Features)};
   \node (LP)   [LP, right = 0.7 cm of Latent.north east] {\large Label predictor \\\footnotesize FC(2)+BN+softmax};
    \node (DC)   [DC, right = 0.7 cm of Latent.south east] {\large Domain  classifier \\\footnotesize FC(1)+BN+sigmoid};
    \node (y)   [yd, right = 0.5 cm of LP] {\footnotesize Class label $y$};
    \node (d)   [yd, right = 0.5 cm of DC] {\footnotesize Domain label $d$};
    \node (Ly)   [Ly, above = 0.5 cm of y] {\footnotesize Loss $L_y$};
    \node (Ld)   [Ld, below = 0.5 cm of d] {\footnotesize Loss $L_d$};
    \gettikzxy{(Ly)}{\axy}{\ayy}
    \gettikzxy{(LP.west)}{\axP}{\ayP}
    \node (pLy)[Ly]   at (\axP,\ayy) {\footnotesize $\frac{\partial L_y}{\partial \theta_y}$};
%    \node (pLy)   [Ly, above = 0.1 cm of LP.north west] {\footnotesize $\frac{\partial L_y}{\partial \theta_y}$};
    \gettikzxy{(Ld)}{\axy}{\ayy}
    \gettikzxy{(DC.west)}{\axP}{\ayP}
    \node (pLd)[Ld]   at (\axP,\ayy) {\footnotesize $\frac{\partial L_d}{\partial \theta_d}$};
%     \node (pLd)  [Ld, below = 0.1 cm of DC.south west] {\footnotesize $-\frac{\partial L_d}{\partial \theta_d}$};
     \node (fLy)   [Ly, right = 5cm of LB.north west] {\footnotesize $\frac{\partial L_y}{\partial \theta_f}$};
      \node (fLd)   [Ld, right = 5cm of ULB.south west] {\footnotesize $-\frac{\partial L_d}{\partial \theta_f}$};
     %\node (fLd)   [Ld, below = 0.2 cm of Feature] {\footnotesize $\frac{\partial L_d}{\partial \theta_f}$};
  \draw[
        -triangle 90, gray,
        line width=0.5mm, 
        postaction={draw, line width=3mm, shorten >=2mm, -}
         ]            
    (LB) -- (Feature);
\draw[
        -triangle 90, gray,
        line width=0.5mm, 
        postaction={draw, line width=3mm, shorten >=2mm, -}
         ] 
        (ULB) -- (Feature);
\draw[
        -triangle 90, gray,
        line width=0.5mm, 
        postaction={draw, line width=3mm, shorten >=2mm, -}
         ] 
        (Feature) -- (Latent);
 \draw[
        -triangle 90, gray,
        line width=0.5mm, 
        postaction={draw, line width=3mm, shorten >=2mm, -}
         ] 
        (Latent) -- (LP);
\draw[
        -triangle 90, gray,
        line width=0.5mm, 
        postaction={draw, line width=3mm, shorten >=2mm, -}
         ] 
        (Latent) -- (DC);
 \draw[
        -triangle 90, gray,
        line width=0.5mm, 
        postaction={draw, line width=3mm, shorten >=2mm, -}
         ] 
        (LP) -- (y);
 \draw[
        -triangle 90, gray,
        line width=0.5mm, 
        postaction={draw, line width=3mm, shorten >=2mm, -}
         ] 
        (DC) -- (d);     
 \draw [ line width=0.5mm, blue!60] (Ly) to  [out=180,in=0] (pLy);   
  \draw [ line width=0.5mm, blue!60] (pLy) to  [out=180,in=0] (fLy); 
  \draw[-latex, line width=0.5mm, blue!60] (fLy) to ++(-2.6,0) ;
  
   \draw [ line width=0.5mm, red!60] (Ld) to  [out=180,in=0] (pLd);   
  \draw [ line width=0.5mm, red!60] (pLd) to  [out=180,in=0] (fLd); 
  \draw[-latex, line width=0.5mm, red!60] (fLd) to ++(-2.6,0) ;
  \end{tikzpicture}
  }
  
  
